Parking Behaviour Analysis of Shared E-Bike Users Based on a Real-World Dataset -- A Case Study in Dublin, Ireland

In recent years, an increasing number of shared E-bikes have been rolling out rapidly in our cities. It therefore becomes important to understand new behaviour patterns of the cyclists in using these E-bikes as a foundation for the novel design of shared micromobility services as part of the realisation for next generation intelligent transportation systems. In this paper, we deeply investigate the users' behaviour of shared E-bikes in a case study by using the real-world dataset collected from the shared E-bike company, MOBY, which currently operates in Dublin, Ireland. More specifically, we look into the parking behaviours of users as we know that inappropriate parking of these bikes can not only increase the management costs of the company but also result in other users' inconveniences, especially in situations of battery shortage, which inevitably reduces the overall operational efficacy of these shared E-bikes. Our work has conducted analysis at both bike station and individual level in a fully anonymous and GDPR-Compliant manner, and our results have shown that up to 12.9% of shared E-bike users did not park their bikes properly at the designated stands. Different visualisation tools have been applied to better illustrate our obtained results.

==> sen e-bike paper/table_for_user_and_stand.tex <==
\clearpage
\appendices
\begin{table*}
\caption{User and Stand}
\label{table_01}
\begin{tabularx}{\textwidth}{@{}l*{15}{C}c@{}}
\toprule
User/Stand &    19  &    39  &    49  &    53  &   60  &  89  &    104 &    116 &    129 &    155 &    158 &    190 &    218 &    252 &     262 \\
\midrule
2276 &      - &      0 &      - &    100 &     - &    - &      0 &      - &      - &    100 &      - &    100 &      - &      - &       - \\
2277 &    100 &    100 &      - &      - &  87.5 &    - &      - &      - &  99.99 &    100 &      - &    100 &    100 &      - &   69.66 \\
2297 &      0 &      - &      - &      - &     - &    - &      - &      - &      - &      - &      - &      - &      - &      - &       0 \\
2305 &      - &      - &      - &      - &   100 &    - &      - &      - &      - &      - &      - &      - &      - &      - &   86.34 \\
2376 &      - &      - &    100 &      - &     - &    - &      - &      - &      - &      - &      - &      - &      - &      - &       - \\
2493 &      - &      - &      - &      - &     - &    - &      - &      - &      - &      - &      - &      - &      - &      - &       - \\
2504 &     50 &      - &      - &      - &     - &    - &      - &      - &  83.32 &      - &      - &   87.5 &      - &      0 &       0 \\
2529 &      - &  66.66 &      - &      - &     - &    - &      - &      - &      - &      - &      - &      - &      - &      - &       0 \\
2560 &  72.72 &  28.57 &  57.15 &    100 &     - &  100 &     50 &    100 &    100 &  57.15 &     60 &  66.66 &      - &  54.54 &      60 \\
2565 &      - &      - &      - &      - &     - &    - &      - &      - &      - &      - &      - &      - &      - &      - &     100 \\
2567 &      - &      - &      - &      - &     - &    - &      - &      - &      - &      - &      - &      - &      - &    100 &       - \\
2605 &      - &      - &      - &      - &     - &    - &      - &      - &      - &      - &      - &      - &      - &      - &       - \\
2622 &     60 &      0 &      - &      - &     - &    - &      - &      - &      - &      - &      - &      - &      - &      - &       - \\
2632 &      - &      - &      - &      - &     - &    - &      - &      - &      - &      - &      - &      - &      - &      - &       - \\
2637 &      - &      - &      - &      - &     - &    - &      - &      - &      - &    100 &      - &      - &      - &      - &       - \\
2819 &    100 &    100 &      - &      - &   100 &    - &     50 &      - &      - &  86.68 &      - &      - &      - &     50 &   33.34 \\
3691 &      - &      - &      - &      - &     - &    - &      - &      - &      - &  88.89 &      - &      - &      - &      - &       - \\
3812 &      - &  57.15 &      - &      - &     - &    - &      - &    100 &      - &      - &    100 &      - &      - &      - &       0 \\
3841 &      - &      - &      - &      - &     - &    - &     50 &      - &    100 &  86.72 &      - &      - &      - &     75 &       - \\
3861 &      - &      - &      - &      - &     - &  100 &      - &      - &      - &      - &      - &      - &    100 &     75 &     100 \\
3972 &  14.28 &      - &      - &      - &     - &    - &      - &    100 &      - &      - &      - &  72.76 &      - &      - &       - \\
3996 &      - &      - &      - &      - &   100 &  100 &    100 &      - &      - &  33.34 &      0 &      - &      - &    100 &     100 \\
4132 &      - &    100 &     50 &      - &     - &    0 &      - &      - &      - &      - &      - &      - &      - &     90 &   68.75 \\
4162 &      - &      - &  57.14 &  83.34 &   100 &  100 &      - &      - &      - &      - &      - &      - &      - &      - &   64.29 \\
4194 &      - &      - &      - &      0 &     - &    - &      - &      - &      - &      - &      - &      - &      - &  68.03 &       - \\
4264 &    100 &     75 &      - &      - &     0 &    - &  24.99 &      - &      0 &  82.35 &      0 &      - &      - &      - &   99.99 \\
4356 &    100 &      - &      - &    100 &     - &    - &      - &     50 &      - &      - &      - &      0 &     68 &      - &       - \\
4477 &    100 &      - &      - &      0 &     - &    - &      - &  99.99 &      - &      - &      - &      - &    100 &    100 &     100 \\
4539 &      - &      - &      - &      - &     - &    - &      - &      - &  62.16 &      - &      - &      - &      - &    100 &   85.72 \\
4546 &     60 &      - &      - &    100 &     0 &    - &      - &    100 &      - &      - &      - &      - &  71.43 &    100 &       - \\
4588 &  66.66 &      - &      - &     40 &     - &    - &      - &      - &      - &      - &      - &      - &  64.29 &    100 &       - \\
4848 &      - &      - &    100 &      - &     - &    - &      - &    100 &      - &      - &      - &      - &      - &      - &     100 \\
5035 &      - &      - &      - &      - &     - &    - &      - &      - &    100 &      - &    100 &      - &      - &    100 &     100 \\
5114 &  58.82 &  57.15 &      - &      - &     - &    - &      - &      - &    100 &      - &      - &      - &  66.66 &      - &       - \\
5244 &      - &      - &    100 &      - &     - &    - &      - &      - &  78.37 &      - &      - &      - &      - &    100 &     100 \\
5268 &    100 &    100 &      - &      - &     - &    - &      - &      - &      - &      - &      - &    100 &      - &      0 &     100 \\
5312 &      - &      - &      - &      - &     - &    - &      - &      - &      - &      - &      - &      - &      - &      - &       - \\
5382 &     50 &      - &      0 &      - &     - &    0 &      - &  33.34 &      - &      - &      - &      - &     50 &      - &   42.86 \\
5478 &      - &      - &      - &      - &     - &    - &      - &      - &   77.5 &      - &    100 &      - &      - &    100 &   33.34 \\
5540 &      - &      - &  66.67 &      - &     - &    - &      - &      - &      - &      - &      - &      - &      - &    100 &       - \\
5568 &      - &      - &      - &      - &     - &    - &      - &      - &      - &      - &      - &      - &      - &      0 &       - \\
5664 &      - &      - &      - &      - &     - &    - &      - &      - &      - &      - &      - &      - &      - &      - &  100.01 \\
6020 &    100 &      - &      - &      - &     - &    - &      - &      - &      - &      - &      - &    100 &      - &     60 &       - \\
6084 &      - &      - &      0 &      - &   100 &    - &      - &      - &      - &      - &      - &      - &      - &    100 &       - \\
6104 &    100 &      - &      - &      - &     - &    - &     60 &      - &      - &   84.2 &      - &      0 &      - &  42.86 &       - \\
6168 &      - &      - &     50 &      - &     - &    - &   12.5 &      - &      - &      0 &      - &    100 &      - &      - &      50 \\
6218 &      - &      - &      - &      - &     - &    - &      - &      - &      - &      - &    100 &      - &      - &      - &   49.99 \\
6263 &      - &      - &      - &   61.9 &   100 &    - &      - &      0 &      - &      - &    100 &      - &     50 &      - &       0 \\
6481 &     60 &      - &     50 &      - &     0 &    - &     50 &     50 &      - &      0 &      - &      - &      - &      0 &      40 \\
6628 &      - &      - &      - &      - &     - &    - &      0 &      - &      - &    100 &      - &      - &      - &      - &       - \\
6653 &      - &      - &      - &      - &     - &    - &      - &      - &  77.78 &      - &      - &      - &      - &     75 &       - \\
6690 &      - &    100 &      - &      - &     - &    - &      - &      - &      - &      - &      - &      - &      - &      - &       - \\
6709 &     80 &      - &      - &      - &     - &    - &      - &      - &      - &      - &      - &      - &      - &      - &      80 \\
6717 &      - &      - &      - &      - &     - &    0 &      - &      - &      - &      - &     50 &      - &      - &      - &       - \\
6939 &      - &      - &      - &      - &     - &    - &  90.91 &      - &      - &  72.91 &      - &      - &      - &      - &      75 \\
7187 &      - &      - &      - &      - &     - &    0 &      - &      - &      - &      - &      - &      - &      - &  41.67 &       - \\
7409 &      - &      - &      - &      - &     - &    - &  75.01 &      - &      - &  93.75 &      - &      - &      - &      - &       - \\
7424 &      - &    100 &      - &      - &     - &    - &     75 &    100 &      0 &      - &      0 &      - &      - &      - &       - \\
7614 &   65.3 &     50 &      - &      - &     - &    - &      - &      - &      - &      - &      - &      - &      0 &      - &     100 \\
7650 &      0 &      - &  66.67 &      - &     0 &  100 &      - &      - &      - &      - &     50 &      - &      - &      - &     100 \\
7906 &      - &      - &      - &      - &     - &    0 &      - &      - &      - &      - &      - &      - &      - &      - &   66.67 \\
8322 &      0 &      - &    100 &    100 &     - &    - &      - &      - &      - &      - &  66.68 &      - &  68.75 &      - &       - \\
8507 &      - &      - &      - &      - &     - &    - &  99.99 &      - &      - &  78.93 &  76.47 &      - &      - &    100 &       - \\
\bottomrule
\end{tabularx}
\end{table*}

\begin{table*}
\caption{User and Stand}
\label{table_02}
\begin{tabularx}{\textwidth}{@{}l*{15}{C}c@{}}
\toprule
User/Stand &    282 &    304 &    305 &    313 &    319 &    330 &    333 &    349 &    363 &    454 &    476 &    496 &    506 &    545 &    546 \\
\midrule
2276 &      - &      - &      - &      - &      - &      - &      - &      - &    100 &    100 &    100 &      - &      - &  66.67 &      0 \\
2277 &  71.44 &      - &      - &     50 &  99.99 &      0 &    100 &    100 &      - &  42.86 &    100 &      - &      - &      - &      - \\
2297 &      - &      - &      - &      - &    100 &      - &      - &      - &      - &      - &      - &      - &      - &    100 &      - \\
2305 &      - &      - &      - &    100 &      - &      - &      - &    100 &      - &    100 &      - &      - &      - &      - &      - \\
2376 &      - &      - &      - &      - &    100 &      - &      - &      - &      - &      - &      - &      - &      - &      - &    100 \\
2493 &      0 &      - &      - &      - &      - &      - &      - &      - &      - &      0 &      - &      - &      - &      - &      - \\
2504 &      - &      - &      - &      - &      - &      - &      - &      - &    100 &      - &      - &      - &      - &   87.5 &      - \\
2529 &      - &      - &     25 &      - &      - &      - &      - &      - &      - &    100 &      - &      - &      - &      - &      - \\
2560 &     40 &  33.33 &  71.44 &  66.68 &  68.58 &    100 &  66.68 &      0 &      0 &   62.5 &  83.32 &    100 &  61.89 &  61.11 &    100 \\
2565 &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - \\
2567 &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &    100 \\
2605 &      - &      - &      - &  44.44 &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &    100 \\
2622 &      - &      - &      - &      - &      - &      - &  33.33 &      - &      - &      - &      - &      - &      - &      - &      - \\
2632 &      - &      - &      - &      - &      - &      - &      - &      - &      - &      0 &      - &      - &      - &      - &      - \\
2637 &  72.72 &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - \\
2819 &    100 &      - &      - &      - &      - &      - &      - &      - &      - &    100 &    100 &    100 &      - &      0 &      - \\
3691 &    100 &      - &      - &      - &     80 &      - &      - &      - &  83.34 &      - &      - &      - &  82.26 &  88.89 &      - \\
3812 &      - &  65.79 &     50 &      - &      - &      - &      - &    100 &      - &      - &      - &      0 &      - &  73.08 &      - \\
3841 &      0 &      - &      - &      - &    100 &      - &      - &      - &      - &      - &      - &      - &      0 &  71.43 &    100 \\
3861 &      - &      - &      - &      - &      - &      - &      - &      - &    100 &      - &      - &      - &      - &  83.33 &      - \\
3972 &    100 &    100 &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - \\
3996 &    100 &      - &      - &      - &      - &      - &      - &    100 &  99.99 &    100 &      - &     50 &      - &     50 &      - \\
4132 &      - &      - &  83.78 &      - &    100 &    100 &     80 &      - &      - &      - &     80 &      - &      - &      - &    100 \\
4162 &      - &      - &      - &      - &      - &      - &      - &      - &      - &    100 &      - &      - &      - &     50 &  74.06 \\
4194 &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &     50 &      - &      - &      - &      - \\
4264 &  73.33 &    100 &      - &      - &    100 &      - &      - &      - &      - &      - &      - &      - &      - &  77.79 &      - \\
4356 &      - &    100 &     25 &      - &      - &    100 &  66.67 &      - &      - &    100 &      - &      0 &      - &      - &    100 \\
4477 &      - &  52.93 &    100 &    100 &      - &      - &      - &    100 &      0 &      - &      - &      0 &      - &      0 &      - \\
4539 &      - &      - &  66.67 &      - &      - &    100 &      - &      - &      - &      - &      - &    100 &      - &      - &      0 \\
4546 &      - &      - &  80.32 &      - &      - &      - &      - &      - &      - &      - &      - &  92.31 &      - &      - &      - \\
4588 &      - &      - &   70.2 &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - \\
4848 &      - &      - &    100 &      - &      - &      - &      0 &      - &    100 &      - &      - &    100 &      - &      0 &      - \\
5035 &    100 &  66.67 &      - &      - &      0 &  72.72 &    100 &     50 &      - &      - &    100 &      - &      - &     50 &      - \\
5114 &      - &      - &  33.33 &      - &      - &      - &    100 &      - &      - &      - &      - &      - &      - &      - &      - \\
5244 &      - &      - &      - &    100 &  78.13 &      - &      - &      - &      - &      - &      0 &      - &    100 &      - &    100 \\
5268 &      - &      - &  66.66 &      - &      - &    100 &     70 &      - &      - &      - &      - &      - &    100 &      - &      - \\
5312 &      - &      - &      - &      - &      - &    100 &      - &      - &      - &      - &      - &      - &      - &      - &      - \\
5382 &      - &  60.01 &      - &      - &      - &      - &      - &      - &      - &      - &      - &      0 &      - &      - &      0 \\
5478 &      - &      - &      - &      - &      - &      - &      - &      - &      - &    100 &      - &      - &      - &      - &      - \\
5540 &      - &      - &      - &     50 &  88.88 &      - &      - &      - &      - &      - &      - &      - &      - &  33.33 &  82.62 \\
5568 &      - &      - &      - &      - &      - &   96.3 &     60 &      - &    100 &      - &      - &    100 &      - &  82.34 &    100 \\
5664 &      - &      - &      - &      - &      - &      - &      - &      - &      - &    100 &      - &      - &      - &    100 &      - \\
6020 &      - &      - &      - &      - &      - &    100 &     75 &      - &      - &      - &      - &      - &      - &     60 &     50 \\
6084 &    100 &      - &      0 &   62.5 &  65.48 &    100 &     75 &      - &      - &      0 &      - &      - &     75 &     75 &     50 \\
6104 &  66.67 &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      0 &     50 &      - &      - \\
6168 &    100 &      - &      - &    100 &  66.66 &      - &      - &      - &    100 &      - &      - &      - &      - &  99.99 &     50 \\
6218 &      - &      - &      - &  66.68 &  59.53 &      - &      - &  33.34 &      - &      - &      - &      - &      0 &      - &      - \\
6263 &      - &  33.33 &    100 &      - &      - &      - &      - &      0 &      - &      - &      - &      - &      - &      - &      - \\
6481 &  34.55 &      - &      - &  67.74 &  47.05 &      - &      - &      - &    100 &    100 &      - &      - &  71.44 &  57.77 &      - \\
6628 &  78.06 &      - &      - &  83.34 &  66.66 &      - &      - &      - &    100 &      - &      - &      - &      - &  90.92 &      0 \\
6653 &      - &      - &      - &      - &      - &      - &      - &      - &      - &    100 &      0 &      - &      - &      - &      - \\
6690 &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - \\
6709 &      - &      - &      - &      - &      - &      - &    100 &      - &      - &      - &      - &      - &      - &      - &      - \\
6717 &    100 &    100 &      - &      - &      - &      - &      - &      - &      - &      0 &      - &  57.15 &      - &    100 &      - \\
6939 &     75 &      - &      - &      - &      - &      - &      - &   62.5 &    100 &      - &      - &    100 &      - &      - &      - \\
7187 &    100 &      - &  60.24 &      - &      - &      - &     50 &      - &     80 &      - &  66.67 &    100 &      - &      - &      - \\
7409 &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - \\
7424 &      - &      - &    100 &      - &      0 &      - &      - &      - &      0 &  66.66 &      - &    100 &      0 &      - &      - \\
7614 &    100 &      0 &  77.78 &      - &      - &      - &    100 &      - &      - &      - &      - &      - &      - &      - &      - \\
7650 &      - &      0 &     75 &   69.8 &  66.68 &    100 &      0 &      - &      - &      - &    100 &    100 &     80 &    100 &     75 \\
7906 &     70 &      - &      - &      - &      - &      - &      - &      - &      - &      - &      0 &      0 &      - &      - &      - \\
8322 &    100 &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &    100 &      - &    100 &     75 \\
8507 &  33.33 &      - &      - &      - &    100 &      - &      - &      - &      - &      - &     50 &      - &      - &      0 &    100 \\
\bottomrule
\end{tabularx}
\end{table*}

\begin{table*}
\caption{User and Stand}
\label{table_03}
\begin{tabularx}{\textwidth}{@{}l*{15}{C}c@{}}
\toprule
User/Stand &    554 &    571 &     572 &    659 &    669 &    695 &    705 &    716 &  774 &    778 &    788 &    798 &    843 &    858 &    865 \\
\midrule
2276 &     50 &      0 &       0 &      - &  57.14 &    100 &      - &    100 &    - &      0 &      - &      - &      - &      - &      - \\
2277 &     60 &    100 &  100.01 &    100 &  92.84 &      - &    100 &     50 &    - &      - &    100 &      - &  42.86 &      - &     50 \\
2297 &      - &      - &       - &      0 &      0 &      - &      - &      - &    - &      - &      - &      - &      - &      - &      - \\
2305 &      - &    100 &     100 &      - &    100 &      - &    100 &     50 &    - &      - &      - &    100 &      - &      - &    100 \\
2376 &      - &      - &       - &      - &      - &      - &      - &      - &    - &     50 &      - &      - &      - &      - &      - \\
2493 &     50 &      - &       - &      - &  66.66 &      - &      - &      - &    0 &      - &    100 &      - &      - &      - &      - \\
2504 &  92.76 &      0 &     100 &      - &      - &      - &      - &      - &  100 &  66.66 &      - &      - &      - &      - &  84.62 \\
2529 &      - &      - &       - &      - &      - &      - &      - &      - &    - &      - &      - &      - &      - &      - &      - \\
2560 &  77.25 &      - &   83.35 &  44.46 &  66.17 &  42.86 &    100 &      - &   80 &   85.7 &  99.99 &     40 &      0 &      0 &    100 \\
2565 &      - &      - &       - &      - &      - &      - &      - &      - &    - &      - &      - &      - &      - &      - &      - \\
2567 &      - &      - &       - &      - &      - &      - &      - &      - &    - &      - &      - &      - &      - &      - &      - \\
2605 &      - &      - &       - &      - &      - &      - &      - &      - &    - &      - &      - &      - &      - &      - &      - \\
2622 &      - &      - &       - &      - &      - &      - &      - &      0 &    - &      - &      - &      - &      - &      - &      - \\
2632 &      - &      - &       - &      - &      - &      - &      - &    100 &    - &      - &      - &      - &      - &      - &      - \\
2637 &      - &      - &       - &      - &      - &      - &      - &      - &    - &      - &      - &      - &      - &      - &      - \\
2819 &      0 &    100 &     100 &      - &      - &      - &    100 &      - &    0 &      - &      - &  99.99 &  66.66 &      - &      - \\
3691 &     75 &      - &   88.89 &     75 &      - &      - &      - &      - &   80 &    100 &      - &      - &      - &      - &      - \\
3812 &  68.75 &  66.67 &       - &      - &      - &      - &      - &      0 &    - &  88.89 &    100 &      - &     50 &      - &    100 \\
3841 &    100 &      - &       - &  82.15 &      - &      - &      - &      - &  100 &  83.34 &      - &      - &      - &      0 &      - \\
3861 &    100 &      - &   55.56 &  81.81 &      - &      - &    100 &    100 &    - &    100 &      - &      - &    100 &      - &      - \\
3972 &      - &    100 &     100 &      - &    100 &     50 &      - &      - &    - &    100 &  71.43 &      - &    100 &      - &      - \\
3996 &    100 &  57.15 &     100 &  33.34 &      - &      - &    100 &      - &  100 &     60 &    100 &    100 &    100 &      - &      - \\
4132 &      - &      - &     100 &      - &      - &      - &      - &    100 &    - &  33.34 &      0 &      - &    100 &    100 &    100 \\
4162 &      - &      - &   46.15 &      - &      - &      - &      0 &     50 &    - &      - &      - &  73.78 &    100 &     75 &      - \\
4194 &      - &      - &       - &      - &      - &      - &      - &      - &    - &      - &     50 &     75 &      0 &      - &      - \\
4264 &    100 &      - &       - &      - &      - &      - &      - &    100 &    - &     60 &    100 &      - &      - &      - &      - \\
4356 &      - &     50 &     100 &      - &      - &      - &     50 &      - &    - &      - &  83.35 &  71.43 &  66.66 &      - &      - \\
4477 &      - &   87.5 &     100 &    100 &      - &      - &    100 &    100 &    - &      - &  75.03 &    100 &     50 &      - &      - \\
4539 &      - &      - &       - &      - &      - &    100 &      - &      - &   50 &      - &      - &      - &      - &      - &      - \\
4546 &      - &      - &       - &      - &      - &    100 &    100 &      - &    - &      - &  99.99 &    100 &     80 &      - &      - \\
4588 &      - &      - &       - &      - &      - &      - &      - &      - &    - &      - &    100 &  86.67 &    100 &      - &      - \\
4848 &      - &    100 &       - &      - &      - &      - &      - &      - &    - &    100 &    100 &      0 &    100 &  66.66 &      - \\
5035 &  61.55 &  99.99 &     100 &    100 &      - &      - &  33.33 &  33.33 &  100 &    100 &    100 &      - &     60 &      - &      - \\
5114 &      - &      - &       - &      - &      - &      - &      - &      - &    - &      - &     20 &    100 &      0 &      - &    100 \\
5244 &      - &      - &       - &      - &      - &     75 &      - &      - &  100 &    100 &      - &      - &    100 &      - &      - \\
5268 &      - &    100 &       - &      - &      - &      - &      - &      - &    - &      - &    100 &      - &    100 &      - &    100 \\
5312 &      - &    100 &       - &      - &      - &      - &      - &      0 &    - &      - &      - &      - &      - &      - &      - \\
5382 &      - &    100 &   71.43 &      - &      - &      - &    100 &    100 &    - &      - &  44.43 &      - &      - &      0 &      - \\
5478 &      - &      - &   85.72 &    100 &      - &      - &    100 &      - &    0 &     75 &      - &      0 &      - &      - &      - \\
5540 &      - &      - &       - &    100 &      - &      - &    100 &      - &  100 &      - &      - &      - &      - &  88.23 &      - \\
5568 &      0 &      - &     100 &      - &      - &      - &      - &      - &    - &  57.14 &      - &      - &      - &      - &      - \\
5664 &      - &      - &   99.99 &      - &      - &  95.35 &      - &    100 &    - &     50 &      - &      - &      - &      - &      - \\
6020 &  66.67 &      - &     100 &      - &      - &      - &      - &    100 &    - &    100 &      - &      - &      - &      - &      - \\
6084 &    100 &      0 &     100 &      - &      - &      - &      - &     50 &    - &    100 &      - &      - &      0 &      - &     50 \\
6104 &      - &      - &       - &  33.34 &      - &      - &    100 &    100 &    - &    100 &      - &      - &      - &      - &    100 \\
6168 &  58.32 &      - &       - &    100 &      - &      - &      - &      0 &    - &    100 &      - &      0 &      - &    100 &      - \\
6218 &      - &      - &   85.72 &      - &      - &      - &    100 &     70 &  100 &    100 &      - &      - &    100 &      - &      - \\
6263 &      - &    100 &       - &      - &      - &      - &    100 &      - &    - &  66.66 &    100 &  48.14 &    100 &      - &      - \\
6481 &  55.38 &      - &      50 &      - &    100 &      - &      - &    100 &    0 &  54.71 &      - &      - &     50 &     75 &      0 \\
6628 &  33.33 &      - &       - &      - &      - &      - &      - &      - &    - &  66.66 &      - &      - &    100 &    100 &      - \\
6653 &      - &      - &       0 &      - &      - &  65.87 &      - &      - &    - &      - &      - &      - &      - &      - &      - \\
6690 &      - &      - &       - &      - &      - &      - &      - &      - &    - &      - &      - &      - &      - &      - &      - \\
6709 &      - &      0 &       - &    100 &     50 &      - &    100 &      0 &    0 &      - &      0 &      - &    100 &      - &      - \\
6717 &  67.01 &      - &     100 &    100 &      - &      - &      - &      0 &    - &  66.66 &      - &      - &    100 &      0 &      - \\
6939 &      - &      - &     100 &    100 &      - &      - &  66.66 &  63.65 &    - &     50 &      - &      - &      0 &      - &      - \\
7187 &      - &      - &       0 &      - &      - &      - &      - &      - &    - &     80 &      - &      - &    100 &      - &      - \\
7409 &    100 &      - &       - &      - &      - &      - &      - &      - &    - &      - &      - &      - &      - &      - &      - \\
7424 &    100 &      - &       - &      - &   84.2 &    100 &      - &      - &    0 &      - &      - &      - &      - &      0 &      - \\
7614 &      - &      - &       - &      - &      - &     80 &      - &      - &    - &     50 &      0 &      - &      - &      - &      - \\
7650 &    100 &      - &       0 &      - &      - &      - &      - &    100 &    - &  57.14 &      - &      - &     60 &    100 &      - \\
7906 &      - &    100 &      80 &      - &   84.6 &      - &  33.34 &  99.99 &    - &     25 &      - &   64.7 &  83.33 &      - &      - \\
8322 &     40 &      - &       - &      0 &  69.22 &      - &      - &      - &  100 &     75 &     50 &    100 &    100 &      - &      0 \\
8507 &  65.22 &      - &     100 &      - &      - &      - &      - &      - &    - &  33.33 &      - &      - &      - &      - &      - \\
\bottomrule
\end{tabularx}
\end{table*}

\begin{table*}
\caption{User and Stand}
\label{table_04}
\begin{tabularx}{\textwidth}{@{}l*{15}{C}c@{}}
\toprule
User/Stand &   876  & 883  &   901  &   930  &   937  &   940  & 949  &   996  &   1013 &    1023 &   1149 &   1158 &   1164 \\
\midrule
2276 &      0 &    0 &    100 &      - &  60.58 &      - &    - &      - &    100 &       - &    100 &      - &    100 \\
2277 &    100 &    0 &    100 &      - &  68.54 &      - &    - &      - &    100 &       - &    100 &     50 &    100 \\
2297 &      - &    - &      - &      - &  44.64 &      - &    - &      - &      - &       - &      - &      - &      - \\
2305 &    100 &   75 &     50 &      - &    100 &      - &    - &      - &    100 &       - &      - &     75 &    100 \\
2376 &      - &    - &      - &      - &      - &      - &    - &  59.45 &      - &       - &      - &      - &      - \\
2493 &      - &    - &      0 &      - &  76.03 &      - &    - &      - &      - &       - &      - &    100 &      - \\
2504 &      - &    - &    100 &      - &      - &      - &  100 &      - &      - &       - &      - &      - &      - \\
2529 &      - &    - &      - &      - &      - &      - &    - &      - &      - &       - &      - &      - &      - \\
2560 &    100 &   40 &  66.66 &    100 &  71.28 &     50 &  100 &  74.99 &  83.34 &     100 &     75 &  66.67 &  88.89 \\
2565 &      - &    - &      - &      - &      - &      - &    - &      - &      - &       - &      - &      - &      - \\
2567 &      - &    - &      - &      - &      - &      - &    - &      - &      - &       - &      - &      - &      - \\
2605 &      - &    - &      - &      - &     50 &      - &    - &      - &      - &       - &      - &      - &      - \\
2622 &      - &    - &      - &      - &      - &      - &    - &      - &      - &       - &      - &      - &      - \\
2632 &      - &    - &      - &      - &      - &      - &    - &      - &      - &       - &      - &      - &      - \\
2637 &      - &    - &      - &      - &      - &      - &    - &      - &      - &       - &      - &      - &      - \\
2819 &      - &    - &    100 &     80 &      - &      - &    - &      - &    100 &       - &      - &      - &      - \\
3691 &      - &  100 &      - &      - &      - &    100 &    - &    100 &      - &       - &      - &      - &      - \\
3812 &      - &    - &     75 &      - &      - &      - &    - &      - &      - &   66.67 &      - &    100 &      - \\
3841 &      - &    - &      - &      - &      - &      - &  100 &  77.77 &      - &       - &  66.66 &      - &      - \\
3861 &      - &   50 &      - &      - &      - &      - &  100 &  80.02 &      - &       - &      - &      - &      - \\
3972 &      - &    - &      - &      - &      - &      - &    - &      - &      - &       - &      - &      - &      - \\
3996 &    100 &  100 &      - &      - &      - &    100 &    - &  51.72 &      - &       - &      0 &      - &      - \\
4132 &      - &   50 &      - &      - &      - &      - &  100 &      - &      - &  100.01 &    100 &      - &  73.53 \\
4162 &      - &    - &      - &     80 &      - &      - &    - &      - &      - &       - &      - &      - &      - \\
4194 &      - &    - &      - &  84.22 &      - &      - &    - &      - &      - &     100 &  99.99 &      - &      - \\
4264 &      - &    - &     50 &    100 &      - &    100 &    - &      - &      - &       - &    100 &     50 &      - \\
4356 &      - &    - &     50 &    100 &      - &      - &    - &      - &      - &   33.33 &      - &      - &      0 \\
4477 &      - &    - &      - &      0 &      - &      0 &    - &      - &      - &       0 &      - &      - &      - \\
4539 &      - &  100 &    100 &      - &      - &      - &  100 &      - &      - &       - &      - &      0 &  66.21 \\
4546 &      - &    - &      - &    100 &      - &      - &    - &      - &      - &   99.99 &      - &      - &      - \\
4588 &      - &    - &      - &      - &      - &      - &    - &      - &      - &     100 &      - &      - &      - \\
4848 &      - &  100 &      0 &  33.33 &      - &      - &  100 &      - &     68 &       - &      - &      - &    100 \\
5035 &    100 &  100 &      - &  66.65 &      - &      - &    - &      - &      - &       - &      - &    100 &      - \\
5114 &      - &    - &  68.57 &      - &      - &      - &    - &      - &      - &     100 &      - &      - &    100 \\
5244 &      - &    - &      - &      - &      - &    100 &    - &      - &      - &       - &     75 &    100 &      - \\
5268 &      - &  100 &     50 &      - &      - &      - &    - &      - &    100 &     100 &      - &      - &    100 \\
5312 &      - &    - &      - &      - &      - &      - &    - &      - &  76.47 &       - &      - &      - &    100 \\
5382 &      - &   80 &      - &      - &      - &      - &    - &      - &      - &       - &      - &  33.34 &      - \\
5478 &  67.86 &    - &      - &      - &      - &      - &    - &      - &      - &       - &      0 &      - &      - \\
5540 &      - &    - &      - &      - &      - &  83.34 &    - &      - &      - &       - &      - &      - &    100 \\
5568 &      - &    - &      - &      - &      - &      - &    - &      - &      - &   85.71 &      - &      - &    100 \\
5664 &    100 &    - &      - &    100 &      - &      - &    - &      - &      - &       - &      - &    100 &      - \\
6020 &      - &    - &  66.67 &      - &      - &  57.14 &    - &      - &      - &       - &      - &      - &      - \\
6084 &      - &    0 &  62.81 &      0 &      - &     50 &  100 &      - &      - &       - &    100 &      - &  57.14 \\
6104 &      - &    0 &      - &      - &      - &      - &  100 &     50 &      - &       - &     50 &      - &      - \\
6168 &      - &    - &      - &      - &      - &      - &    - &      - &      - &       - &      - &      - &      - \\
6218 &      - &   40 &      - &      - &      - &    100 &    - &      - &      - &       - &      - &      0 &      - \\
6263 &      - &    - &    100 &      - &      - &      - &  100 &      - &      - &       0 &      - &      - &      - \\
6481 &    100 &   50 &      0 &  33.33 &      - &  61.89 &    0 &     80 &      - &       - &     50 &     50 &      - \\
6628 &      - &    - &     50 &      - &      - &    100 &    - &      - &      - &       - &      - &     50 &      - \\
6653 &  99.99 &    - &      - &      - &      - &      - &    0 &      - &      - &       - &      - &      - &    100 \\
6690 &      - &    - &  66.66 &      - &      - &      - &    - &      - &  53.34 &       - &      - &      - &      - \\
6709 &      - &    - &      - &    100 &      - &      - &    - &    100 &      - &       - &      - &  64.28 &      - \\
6717 &      - &    - &      - &      - &      - &      - &    - &      - &      - &       - &      - &      - &      - \\
6939 &      - &   75 &      - &      - &      - &    100 &    - &      - &      - &       - &      - &      - &      - \\
7187 &      - &   60 &      - &      - &      - &      - &    - &      - &      - &      50 &      - &      - &  68.42 \\
7409 &      - &    - &      - &      - &      - &      - &    - &    100 &      - &       - &      - &      - &      - \\
7424 &     50 &    0 &  66.66 &      - &  69.38 &    100 &    - &     50 &  33.34 &     100 &      - &      - &      - \\
7614 &      - &    0 &  68.43 &      - &      - &      - &    - &      - &      - &       - &      - &      - &      - \\
7650 &      - &  100 &      - &      - &      - &      - &    - &      - &      - &       - &      - &      - &      - \\
7906 &      0 &   50 &      - &  76.47 &  86.41 &      - &    - &     50 &      - &       - &     50 &  66.66 &      0 \\
8322 &      - &  100 &      - &      - &  79.22 &      - &    - &      - &      0 &       - &    100 &      - &      - \\
8507 &      - &    - &      - &      - &      - &      - &    - &      - &      - &       - &      0 &      - &      - \\
\bottomrule
\end{tabularx}
\end{table*}

==> table_for_user_and_stand.tex <==
\clearpage
\appendices
\begin{table*}
\caption{User and Stand}
\label{table_01}
\begin{tabularx}{\textwidth}{@{}l*{15}{C}c@{}}
\toprule
User/Stand &    19  &    39  &    49  &    53  &   60  &  89  &    104 &    116 &    129 &    155 &    158 &    190 &    218 &    252 &     262 \\
\midrule
2276 &      - &      0 &      - &    100 &     - &    - &      0 &      - &      - &    100 &      - &    100 &      - &      - &       - \\
2277 &    100 &    100 &      - &      - &  87.5 &    - &      - &      - &  99.99 &    100 &      - &    100 &    100 &      - &   69.66 \\
2297 &      0 &      - &      - &      - &     - &    - &      - &      - &      - &      - &      - &      - &      - &      - &       0 \\
2305 &      - &      - &      - &      - &   100 &    - &      - &      - &      - &      - &      - &      - &      - &      - &   86.34 \\
2376 &      - &      - &    100 &      - &     - &    - &      - &      - &      - &      - &      - &      - &      - &      - &       - \\
2493 &      - &      - &      - &      - &     - &    - &      - &      - &      - &      - &      - &      - &      - &      - &       - \\
2504 &     50 &      - &      - &      - &     - &    - &      - &      - &  83.32 &      - &      - &   87.5 &      - &      0 &       0 \\
2529 &      - &  66.66 &      - &      - &     - &    - &      - &      - &      - &      - &      - &      - &      - &      - &       0 \\
2560 &  72.72 &  28.57 &  57.15 &    100 &     - &  100 &     50 &    100 &    100 &  57.15 &     60 &  66.66 &      - &  54.54 &      60 \\
2565 &      - &      - &      - &      - &     - &    - &      - &      - &      - &      - &      - &      - &      - &      - &     100 \\
2567 &      - &      - &      - &      - &     - &    - &      - &      - &      - &      - &      - &      - &      - &    100 &       - \\
2605 &      - &      - &      - &      - &     - &    - &      - &      - &      - &      - &      - &      - &      - &      - &       - \\
2622 &     60 &      0 &      - &      - &     - &    - &      - &      - &      - &      - &      - &      - &      - &      - &       - \\
2632 &      - &      - &      - &      - &     - &    - &      - &      - &      - &      - &      - &      - &      - &      - &       - \\
2637 &      - &      - &      - &      - &     - &    - &      - &      - &      - &    100 &      - &      - &      - &      - &       - \\
2819 &    100 &    100 &      - &      - &   100 &    - &     50 &      - &      - &  86.68 &      - &      - &      - &     50 &   33.34 \\
3691 &      - &      - &      - &      - &     - &    - &      - &      - &      - &  88.89 &      - &      - &      - &      - &       - \\
3812 &      - &  57.15 &      - &      - &     - &    - &      - &    100 &      - &      - &    100 &      - &      - &      - &       0 \\
3841 &      - &      - &      - &      - &     - &    - &     50 &      - &    100 &  86.72 &      - &      - &      - &     75 &       - \\
3861 &      - &      - &      - &      - &     - &  100 &      - &      - &      - &      - &      - &      - &    100 &     75 &     100 \\
3972 &  14.28 &      - &      - &      - &     - &    - &      - &    100 &      - &      - &      - &  72.76 &      - &      - &       - \\
3996 &      - &      - &      - &      - &   100 &  100 &    100 &      - &      - &  33.34 &      0 &      - &      - &    100 &     100 \\
4132 &      - &    100 &     50 &      - &     - &    0 &      - &      - &      - &      - &      - &      - &      - &     90 &   68.75 \\
4162 &      - &      - &  57.14 &  83.34 &   100 &  100 &      - &      - &      - &      - &      - &      - &      - &      - &   64.29 \\
4194 &      - &      - &      - &      0 &     - &    - &      - &      - &      - &      - &      - &      - &      - &  68.03 &       - \\
4264 &    100 &     75 &      - &      - &     0 &    - &  24.99 &      - &      0 &  82.35 &      0 &      - &      - &      - &   99.99 \\
4356 &    100 &      - &      - &    100 &     - &    - &      - &     50 &      - &      - &      - &      0 &     68 &      - &       - \\
4477 &    100 &      - &      - &      0 &     - &    - &      - &  99.99 &      - &      - &      - &      - &    100 &    100 &     100 \\
4539 &      - &      - &      - &      - &     - &    - &      - &      - &  62.16 &      - &      - &      - &      - &    100 &   85.72 \\
4546 &     60 &      - &      - &    100 &     0 &    - &      - &    100 &      - &      - &      - &      - &  71.43 &    100 &       - \\
4588 &  66.66 &      - &      - &     40 &     - &    - &      - &      - &      - &      - &      - &      - &  64.29 &    100 &       - \\
4848 &      - &      - &    100 &      - &     - &    - &      - &    100 &      - &      - &      - &      - &      - &      - &     100 \\
5035 &      - &      - &      - &      - &     - &    - &      - &      - &    100 &      - &    100 &      - &      - &    100 &     100 \\
5114 &  58.82 &  57.15 &      - &      - &     - &    - &      - &      - &    100 &      - &      - &      - &  66.66 &      - &       - \\
5244 &      - &      - &    100 &      - &     - &    - &      - &      - &  78.37 &      - &      - &      - &      - &    100 &     100 \\
5268 &    100 &    100 &      - &      - &     - &    - &      - &      - &      - &      - &      - &    100 &      - &      0 &     100 \\
5312 &      - &      - &      - &      - &     - &    - &      - &      - &      - &      - &      - &      - &      - &      - &       - \\
5382 &     50 &      - &      0 &      - &     - &    0 &      - &  33.34 &      - &      - &      - &      - &     50 &      - &   42.86 \\
5478 &      - &      - &      - &      - &     - &    - &      - &      - &   77.5 &      - &    100 &      - &      - &    100 &   33.34 \\
5540 &      - &      - &  66.67 &      - &     - &    - &      - &      - &      - &      - &      - &      - &      - &    100 &       - \\
5568 &      - &      - &      - &      - &     - &    - &      - &      - &      - &      - &      - &      - &      - &      0 &       - \\
5664 &      - &      - &      - &      - &     - &    - &      - &      - &      - &      - &      - &      - &      - &      - &  100.01 \\
6020 &    100 &      - &      - &      - &     - &    - &      - &      - &      - &      - &      - &    100 &      - &     60 &       - \\
6084 &      - &      - &      0 &      - &   100 &    - &      - &      - &      - &      - &      - &      - &      - &    100 &       - \\
6104 &    100 &      - &      - &      - &     - &    - &     60 &      - &      - &   84.2 &      - &      0 &      - &  42.86 &       - \\
6168 &      - &      - &     50 &      - &     - &    - &   12.5 &      - &      - &      0 &      - &    100 &      - &      - &      50 \\
6218 &      - &      - &      - &      - &     - &    - &      - &      - &      - &      - &    100 &      - &      - &      - &   49.99 \\
6263 &      - &      - &      - &   61.9 &   100 &    - &      - &      0 &      - &      - &    100 &      - &     50 &      - &       0 \\
6481 &     60 &      - &     50 &      - &     0 &    - &     50 &     50 &      - &      0 &      - &      - &      - &      0 &      40 \\
6628 &      - &      - &      - &      - &     - &    - &      0 &      - &      - &    100 &      - &      - &      - &      - &       - \\
6653 &      - &      - &      - &      - &     - &    - &      - &      - &  77.78 &      - &      - &      - &      - &     75 &       - \\
6690 &      - &    100 &      - &      - &     - &    - &      - &      - &      - &      - &      - &      - &      - &      - &       - \\
6709 &     80 &      - &      - &      - &     - &    - &      - &      - &      - &      - &      - &      - &      - &      - &      80 \\
6717 &      - &      - &      - &      - &     - &    0 &      - &      - &      - &      - &     50 &      - &      - &      - &       - \\
6939 &      - &      - &      - &      - &     - &    - &  90.91 &      - &      - &  72.91 &      - &      - &      - &      - &      75 \\
7187 &      - &      - &      - &      - &     - &    0 &      - &      - &      - &      - &      - &      - &      - &  41.67 &       - \\
7409 &      - &      - &      - &      - &     - &    - &  75.01 &      - &      - &  93.75 &      - &      - &      - &      - &       - \\
7424 &      - &    100 &      - &      - &     - &    - &     75 &    100 &      0 &      - &      0 &      - &      - &      - &       - \\
7614 &   65.3 &     50 &      - &      - &     - &    - &      - &      - &      - &      - &      - &      - &      0 &      - &     100 \\
7650 &      0 &      - &  66.67 &      - &     0 &  100 &      - &      - &      - &      - &     50 &      - &      - &      - &     100 \\
7906 &      - &      - &      - &      - &     - &    0 &      - &      - &      - &      - &      - &      - &      - &      - &   66.67 \\
8322 &      0 &      - &    100 &    100 &     - &    - &      - &      - &      - &      - &  66.68 &      - &  68.75 &      - &       - \\
8507 &      - &      - &      - &      - &     - &    - &  99.99 &      - &      - &  78.93 &  76.47 &      - &      - &    100 &       - \\
\bottomrule
\end{tabularx}
\end{table*}

\begin{table*}
\caption{User and Stand}
\label{table_02}
\begin{tabularx}{\textwidth}{@{}l*{15}{C}c@{}}
\toprule
User/Stand &    282 &    304 &    305 &    313 &    319 &    330 &    333 &    349 &    363 &    454 &    476 &    496 &    506 &    545 &    546 \\
\midrule
2276 &      - &      - &      - &      - &      - &      - &      - &      - &    100 &    100 &    100 &      - &      - &  66.67 &      0 \\
2277 &  71.44 &      - &      - &     50 &  99.99 &      0 &    100 &    100 &      - &  42.86 &    100 &      - &      - &      - &      - \\
2297 &      - &      - &      - &      - &    100 &      - &      - &      - &      - &      - &      - &      - &      - &    100 &      - \\
2305 &      - &      - &      - &    100 &      - &      - &      - &    100 &      - &    100 &      - &      - &      - &      - &      - \\
2376 &      - &      - &      - &      - &    100 &      - &      - &      - &      - &      - &      - &      - &      - &      - &    100 \\
2493 &      0 &      - &      - &      - &      - &      - &      - &      - &      - &      0 &      - &      - &      - &      - &      - \\
2504 &      - &      - &      - &      - &      - &      - &      - &      - &    100 &      - &      - &      - &      - &   87.5 &      - \\
2529 &      - &      - &     25 &      - &      - &      - &      - &      - &      - &    100 &      - &      - &      - &      - &      - \\
2560 &     40 &  33.33 &  71.44 &  66.68 &  68.58 &    100 &  66.68 &      0 &      0 &   62.5 &  83.32 &    100 &  61.89 &  61.11 &    100 \\
2565 &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - \\
2567 &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &    100 \\
2605 &      - &      - &      - &  44.44 &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &    100 \\
2622 &      - &      - &      - &      - &      - &      - &  33.33 &      - &      - &      - &      - &      - &      - &      - &      - \\
2632 &      - &      - &      - &      - &      - &      - &      - &      - &      - &      0 &      - &      - &      - &      - &      - \\
2637 &  72.72 &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - \\
2819 &    100 &      - &      - &      - &      - &      - &      - &      - &      - &    100 &    100 &    100 &      - &      0 &      - \\
3691 &    100 &      - &      - &      - &     80 &      - &      - &      - &  83.34 &      - &      - &      - &  82.26 &  88.89 &      - \\
3812 &      - &  65.79 &     50 &      - &      - &      - &      - &    100 &      - &      - &      - &      0 &      - &  73.08 &      - \\
3841 &      0 &      - &      - &      - &    100 &      - &      - &      - &      - &      - &      - &      - &      0 &  71.43 &    100 \\
3861 &      - &      - &      - &      - &      - &      - &      - &      - &    100 &      - &      - &      - &      - &  83.33 &      - \\
3972 &    100 &    100 &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - \\
3996 &    100 &      - &      - &      - &      - &      - &      - &    100 &  99.99 &    100 &      - &     50 &      - &     50 &      - \\
4132 &      - &      - &  83.78 &      - &    100 &    100 &     80 &      - &      - &      - &     80 &      - &      - &      - &    100 \\
4162 &      - &      - &      - &      - &      - &      - &      - &      - &      - &    100 &      - &      - &      - &     50 &  74.06 \\
4194 &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &     50 &      - &      - &      - &      - \\
4264 &  73.33 &    100 &      - &      - &    100 &      - &      - &      - &      - &      - &      - &      - &      - &  77.79 &      - \\
4356 &      - &    100 &     25 &      - &      - &    100 &  66.67 &      - &      - &    100 &      - &      0 &      - &      - &    100 \\
4477 &      - &  52.93 &    100 &    100 &      - &      - &      - &    100 &      0 &      - &      - &      0 &      - &      0 &      - \\
4539 &      - &      - &  66.67 &      - &      - &    100 &      - &      - &      - &      - &      - &    100 &      - &      - &      0 \\
4546 &      - &      - &  80.32 &      - &      - &      - &      - &      - &      - &      - &      - &  92.31 &      - &      - &      - \\
4588 &      - &      - &   70.2 &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - \\
4848 &      - &      - &    100 &      - &      - &      - &      0 &      - &    100 &      - &      - &    100 &      - &      0 &      - \\
5035 &    100 &  66.67 &      - &      - &      0 &  72.72 &    100 &     50 &      - &      - &    100 &      - &      - &     50 &      - \\
5114 &      - &      - &  33.33 &      - &      - &      - &    100 &      - &      - &      - &      - &      - &      - &      - &      - \\
5244 &      - &      - &      - &    100 &  78.13 &      - &      - &      - &      - &      - &      0 &      - &    100 &      - &    100 \\
5268 &      - &      - &  66.66 &      - &      - &    100 &     70 &      - &      - &      - &      - &      - &    100 &      - &      - \\
5312 &      - &      - &      - &      - &      - &    100 &      - &      - &      - &      - &      - &      - &      - &      - &      - \\
5382 &      - &  60.01 &      - &      - &      - &      - &      - &      - &      - &      - &      - &      0 &      - &      - &      0 \\
5478 &      - &      - &      - &      - &      - &      - &      - &      - &      - &    100 &      - &      - &      - &      - &      - \\
5540 &      - &      - &      - &     50 &  88.88 &      - &      - &      - &      - &      - &      - &      - &      - &  33.33 &  82.62 \\
5568 &      - &      - &      - &      - &      - &   96.3 &     60 &      - &    100 &      - &      - &    100 &      - &  82.34 &    100 \\
5664 &      - &      - &      - &      - &      - &      - &      - &      - &      - &    100 &      - &      - &      - &    100 &      - \\
6020 &      - &      - &      - &      - &      - &    100 &     75 &      - &      - &      - &      - &      - &      - &     60 &     50 \\
6084 &    100 &      - &      0 &   62.5 &  65.48 &    100 &     75 &      - &      - &      0 &      - &      - &     75 &     75 &     50 \\
6104 &  66.67 &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      0 &     50 &      - &      - \\
6168 &    100 &      - &      - &    100 &  66.66 &      - &      - &      - &    100 &      - &      - &      - &      - &  99.99 &     50 \\
6218 &      - &      - &      - &  66.68 &  59.53 &      - &      - &  33.34 &      - &      - &      - &      - &      0 &      - &      - \\
6263 &      - &  33.33 &    100 &      - &      - &      - &      - &      0 &      - &      - &      - &      - &      - &      - &      - \\
6481 &  34.55 &      - &      - &  67.74 &  47.05 &      - &      - &      - &    100 &    100 &      - &      - &  71.44 &  57.77 &      - \\
6628 &  78.06 &      - &      - &  83.34 &  66.66 &      - &      - &      - &    100 &      - &      - &      - &      - &  90.92 &      0 \\
6653 &      - &      - &      - &      - &      - &      - &      - &      - &      - &    100 &      0 &      - &      - &      - &      - \\
6690 &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - \\
6709 &      - &      - &      - &      - &      - &      - &    100 &      - &      - &      - &      - &      - &      - &      - &      - \\
6717 &    100 &    100 &      - &      - &      - &      - &      - &      - &      - &      0 &      - &  57.15 &      - &    100 &      - \\
6939 &     75 &      - &      - &      - &      - &      - &      - &   62.5 &    100 &      - &      - &    100 &      - &      - &      - \\
7187 &    100 &      - &  60.24 &      - &      - &      - &     50 &      - &     80 &      - &  66.67 &    100 &      - &      - &      - \\
7409 &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - \\
7424 &      - &      - &    100 &      - &      0 &      - &      - &      - &      0 &  66.66 &      - &    100 &      0 &      - &      - \\
7614 &    100 &      0 &  77.78 &      - &      - &      - &    100 &      - &      - &      - &      - &      - &      - &      - &      - \\
7650 &      - &      0 &     75 &   69.8 &  66.68 &    100 &      0 &      - &      - &      - &    100 &    100 &     80 &    100 &     75 \\
7906 &     70 &      - &      - &      - &      - &      - &      - &      - &      - &      - &      0 &      0 &      - &      - &      - \\
8322 &    100 &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &    100 &      - &    100 &     75 \\
8507 &  33.33 &      - &      - &      - &    100 &      - &      - &      - &      - &      - &     50 &      - &      - &      0 &    100 \\
\bottomrule
\end{tabularx}
\end{table*}

\begin{table*}
\caption{User and Stand}
\label{table_03}
\begin{tabularx}{\textwidth}{@{}l*{15}{C}c@{}}
\toprule
User/Stand &    554 &    571 &     572 &    659 &    669 &    695 &    705 &    716 &  774 &    778 &    788 &    798 &    843 &    858 &    865 \\
\midrule
2276 &     50 &      0 &       0 &      - &  57.14 &    100 &      - &    100 &    - &      0 &      - &      - &      - &      - &      - \\
2277 &     60 &    100 &  100.01 &    100 &  92.84 &      - &    100 &     50 &    - &      - &    100 &      - &  42.86 &      - &     50 \\
2297 &      - &      - &       - &      0 &      0 &      - &      - &      - &    - &      - &      - &      - &      - &      - &      - \\
2305 &      - &    100 &     100 &      - &    100 &      - &    100 &     50 &    - &      - &      - &    100 &      - &      - &    100 \\
2376 &      - &      - &       - &      - &      - &      - &      - &      - &    - &     50 &      - &      - &      - &      - &      - \\
2493 &     50 &      - &       - &      - &  66.66 &      - &      - &      - &    0 &      - &    100 &      - &      - &      - &      - \\
2504 &  92.76 &      0 &     100 &      - &      - &      - &      - &      - &  100 &  66.66 &      - &      - &      - &      - &  84.62 \\
2529 &      - &      - &       - &      - &      - &      - &      - &      - &    - &      - &      - &      - &      - &      - &      - \\
2560 &  77.25 &      - &   83.35 &  44.46 &  66.17 &  42.86 &    100 &      - &   80 &   85.7 &  99.99 &     40 &      0 &      0 &    100 \\
2565 &      - &      - &       - &      - &      - &      - &      - &      - &    - &      - &      - &      - &      - &      - &      - \\
2567 &      - &      - &       - &      - &      - &      - &      - &      - &    - &      - &      - &      - &      - &      - &      - \\
2605 &      - &      - &       - &      - &      - &      - &      - &      - &    - &      - &      - &      - &      - &      - &      - \\
2622 &      - &      - &       - &      - &      - &      - &      - &      0 &    - &      - &      - &      - &      - &      - &      - \\
2632 &      - &      - &       - &      - &      - &      - &      - &    100 &    - &      - &      - &      - &      - &      - &      - \\
2637 &      - &      - &       - &      - &      - &      - &      - &      - &    - &      - &      - &      - &      - &      - &      - \\
2819 &      0 &    100 &     100 &      - &      - &      - &    100 &      - &    0 &      - &      - &  99.99 &  66.66 &      - &      - \\
3691 &     75 &      - &   88.89 &     75 &      - &      - &      - &      - &   80 &    100 &      - &      - &      - &      - &      - \\
3812 &  68.75 &  66.67 &       - &      - &      - &      - &      - &      0 &    - &  88.89 &    100 &      - &     50 &      - &    100 \\
3841 &    100 &      - &       - &  82.15 &      - &      - &      - &      - &  100 &  83.34 &      - &      - &      - &      0 &      - \\
3861 &    100 &      - &   55.56 &  81.81 &      - &      - &    100 &    100 &    - &    100 &      - &      - &    100 &      - &      - \\
3972 &      - &    100 &     100 &      - &    100 &     50 &      - &      - &    - &    100 &  71.43 &      - &    100 &      - &      - \\
3996 &    100 &  57.15 &     100 &  33.34 &      - &      - &    100 &      - &  100 &     60 &    100 &    100 &    100 &      - &      - \\
4132 &      - &      - &     100 &      - &      - &      - &      - &    100 &    - &  33.34 &      0 &      - &    100 &    100 &    100 \\
4162 &      - &      - &   46.15 &      - &      - &      - &      0 &     50 &    - &      - &      - &  73.78 &    100 &     75 &      - \\
4194 &      - &      - &       - &      - &      - &      - &      - &      - &    - &      - &     50 &     75 &      0 &      - &      - \\
4264 &    100 &      - &       - &      - &      - &      - &      - &    100 &    - &     60 &    100 &      - &      - &      - &      - \\
4356 &      - &     50 &     100 &      - &      - &      - &     50 &      - &    - &      - &  83.35 &  71.43 &  66.66 &      - &      - \\
4477 &      - &   87.5 &     100 &    100 &      - &      - &    100 &    100 &    - &      - &  75.03 &    100 &     50 &      - &      - \\
4539 &      - &      - &       - &      - &      - &    100 &      - &      - &   50 &      - &      - &      - &      - &      - &      - \\
4546 &      - &      - &       - &      - &      - &    100 &    100 &      - &    - &      - &  99.99 &    100 &     80 &      - &      - \\
4588 &      - &      - &       - &      - &      - &      - &      - &      - &    - &      - &    100 &  86.67 &    100 &      - &      - \\
4848 &      - &    100 &       - &      - &      - &      - &      - &      - &    - &    100 &    100 &      0 &    100 &  66.66 &      - \\
5035 &  61.55 &  99.99 &     100 &    100 &      - &      - &  33.33 &  33.33 &  100 &    100 &    100 &      - &     60 &      - &      - \\
5114 &      - &      - &       - &      - &      - &      - &      - &      - &    - &      - &     20 &    100 &      0 &      - &    100 \\
5244 &      - &      - &       - &      - &      - &     75 &      - &      - &  100 &    100 &      - &      - &    100 &      - &      - \\
5268 &      - &    100 &       - &      - &      - &      - &      - &      - &    - &      - &    100 &      - &    100 &      - &    100 \\
5312 &      - &    100 &       - &      - &      - &      - &      - &      0 &    - &      - &      - &      - &      - &      - &      - \\
5382 &      - &    100 &   71.43 &      - &      - &      - &    100 &    100 &    - &      - &  44.43 &      - &      - &      0 &      - \\
5478 &      - &      - &   85.72 &    100 &      - &      - &    100 &      - &    0 &     75 &      - &      0 &      - &      - &      - \\
5540 &      - &      - &       - &    100 &      - &      - &    100 &      - &  100 &      - &      - &      - &      - &  88.23 &      - \\
5568 &      0 &      - &     100 &      - &      - &      - &      - &      - &    - &  57.14 &      - &      - &      - &      - &      - \\
5664 &      - &      - &   99.99 &      - &      - &  95.35 &      - &    100 &    - &     50 &      - &      - &      - &      - &      - \\
6020 &  66.67 &      - &     100 &      - &      - &      - &      - &    100 &    - &    100 &      - &      - &      - &      - &      - \\
6084 &    100 &      0 &     100 &      - &      - &      - &      - &     50 &    - &    100 &      - &      - &      0 &      - &     50 \\
6104 &      - &      - &       - &  33.34 &      - &      - &    100 &    100 &    - &    100 &      - &      - &      - &      - &    100 \\
6168 &  58.32 &      - &       - &    100 &      - &      - &      - &      0 &    - &    100 &      - &      0 &      - &    100 &      - \\
6218 &      - &      - &   85.72 &      - &      - &      - &    100 &     70 &  100 &    100 &      - &      - &    100 &      - &      - \\
6263 &      - &    100 &       - &      - &      - &      - &    100 &      - &    - &  66.66 &    100 &  48.14 &    100 &      - &      - \\
6481 &  55.38 &      - &      50 &      - &    100 &      - &      - &    100 &    0 &  54.71 &      - &      - &     50 &     75 &      0 \\
6628 &  33.33 &      - &       - &      - &      - &      - &      - &      - &    - &  66.66 &      - &      - &    100 &    100 &      - \\
6653 &      - &      - &       0 &      - &      - &  65.87 &      - &      - &    - &      - &      - &      - &      - &      - &      - \\
6690 &      - &      - &       - &      - &      - &      - &      - &      - &    - &      - &      - &      - &      - &      - &      - \\
6709 &      - &      0 &       - &    100 &     50 &      - &    100 &      0 &    0 &      - &      0 &      - &    100 &      - &      - \\
6717 &  67.01 &      - &     100 &    100 &      - &      - &      - &      0 &    - &  66.66 &      - &      - &    100 &      0 &      - \\
6939 &      - &      - &     100 &    100 &      - &      - &  66.66 &  63.65 &    - &     50 &      - &      - &      0 &      - &      - \\
7187 &      - &      - &       0 &      - &      - &      - &      - &      - &    - &     80 &      - &      - &    100 &      - &      - \\
7409 &    100 &      - &       - &      - &      - &      - &      - &      - &    - &      - &      - &      - &      - &      - &      - \\
7424 &    100 &      - &       - &      - &   84.2 &    100 &      - &      - &    0 &      - &      - &      - &      - &      0 &      - \\
7614 &      - &      - &       - &      - &      - &     80 &      - &      - &    - &     50 &      0 &      - &      - &      - &      - \\
7650 &    100 &      - &       0 &      - &      - &      - &      - &    100 &    - &  57.14 &      - &      - &     60 &    100 &      - \\
7906 &      - &    100 &      80 &      - &   84.6 &      - &  33.34 &  99.99 &    - &     25 &      - &   64.7 &  83.33 &      - &      - \\
8322 &     40 &      - &       - &      0 &  69.22 &      - &      - &      - &  100 &     75 &     50 &    100 &    100 &      - &      0 \\
8507 &  65.22 &      - &     100 &      - &      - &      - &      - &      - &    - &  33.33 &      - &      - &      - &      - &      - \\
\bottomrule
\end{tabularx}
\end{table*}

\begin{table*}
\caption{User and Stand}
\label{table_04}
\begin{tabularx}{\textwidth}{@{}l*{15}{C}c@{}}
\toprule
User/Stand &   876  & 883  &   901  &   930  &   937  &   940  & 949  &   996  &   1013 &    1023 &   1149 &   1158 &   1164 \\
\midrule
2276 &      0 &    0 &    100 &      - &  60.58 &      - &    - &      - &    100 &       - &    100 &      - &    100 \\
2277 &    100 &    0 &    100 &      - &  68.54 &      - &    - &      - &    100 &       - &    100 &     50 &    100 \\
2297 &      - &    - &      - &      - &  44.64 &      - &    - &      - &      - &       - &      - &      - &      - \\
2305 &    100 &   75 &     50 &      - &    100 &      - &    - &      - &    100 &       - &      - &     75 &    100 \\
2376 &      - &    - &      - &      - &      - &      - &    - &  59.45 &      - &       - &      - &      - &      - \\
2493 &      - &    - &      0 &      - &  76.03 &      - &    - &      - &      - &       - &      - &    100 &      - \\
2504 &      - &    - &    100 &      - &      - &      - &  100 &      - &      - &       - &      - &      - &      - \\
2529 &      - &    - &      - &      - &      - &      - &    - &      - &      - &       - &      - &      - &      - \\
2560 &    100 &   40 &  66.66 &    100 &  71.28 &     50 &  100 &  74.99 &  83.34 &     100 &     75 &  66.67 &  88.89 \\
2565 &      - &    - &      - &      - &      - &      - &    - &      - &      - &       - &      - &      - &      - \\
2567 &      - &    - &      - &      - &      - &      - &    - &      - &      - &       - &      - &      - &      - \\
2605 &      - &    - &      - &      - &     50 &      - &    - &      - &      - &       - &      - &      - &      - \\
2622 &      - &    - &      - &      - &      - &      - &    - &      - &      - &       - &      - &      - &      - \\
2632 &      - &    - &      - &      - &      - &      - &    - &      - &      - &       - &      - &      - &      - \\
2637 &      - &    - &      - &      - &      - &      - &    - &      - &      - &       - &      - &      - &      - \\
2819 &      - &    - &    100 &     80 &      - &      - &    - &      - &    100 &       - &      - &      - &      - \\
3691 &      - &  100 &      - &      - &      - &    100 &    - &    100 &      - &       - &      - &      - &      - \\
3812 &      - &    - &     75 &      - &      - &      - &    - &      - &      - &   66.67 &      - &    100 &      - \\
3841 &      - &    - &      - &      - &      - &      - &  100 &  77.77 &      - &       - &  66.66 &      - &      - \\
3861 &      - &   50 &      - &      - &      - &      - &  100 &  80.02 &      - &       - &      - &      - &      - \\
3972 &      - &    - &      - &      - &      - &      - &    - &      - &      - &       - &      - &      - &      - \\
3996 &    100 &  100 &      - &      - &      - &    100 &    - &  51.72 &      - &       - &      0 &      - &      - \\
4132 &      - &   50 &      - &      - &      - &      - &  100 &      - &      - &  100.01 &    100 &      - &  73.53 \\
4162 &      - &    - &      - &     80 &      - &      - &    - &      - &      - &       - &      - &      - &      - \\
4194 &      - &    - &      - &  84.22 &      - &      - &    - &      - &      - &     100 &  99.99 &      - &      - \\
4264 &      - &    - &     50 &    100 &      - &    100 &    - &      - &      - &       - &    100 &     50 &      - \\
4356 &      - &    - &     50 &    100 &      - &      - &    - &      - &      - &   33.33 &      - &      - &      0 \\
4477 &      - &    - &      - &      0 &      - &      0 &    - &      - &      - &       0 &      - &      - &      - \\
4539 &      - &  100 &    100 &      - &      - &      - &  100 &      - &      - &       - &      - &      0 &  66.21 \\
4546 &      - &    - &      - &    100 &      - &      - &    - &      - &      - &   99.99 &      - &      - &      - \\
4588 &      - &    - &      - &      - &      - &      - &    - &      - &      - &     100 &      - &      - &      - \\
4848 &      - &  100 &      0 &  33.33 &      - &      - &  100 &      - &     68 &       - &      - &      - &    100 \\
5035 &    100 &  100 &      - &  66.65 &      - &      - &    - &      - &      - &       - &      - &    100 &      - \\
5114 &      - &    - &  68.57 &      - &      - &      - &    - &      - &      - &     100 &      - &      - &    100 \\
5244 &      - &    - &      - &      - &      - &    100 &    - &      - &      - &       - &     75 &    100 &      - \\
5268 &      - &  100 &     50 &      - &      - &      - &    - &      - &    100 &     100 &      - &      - &    100 \\
5312 &      - &    - &      - &      - &      - &      - &    - &      - &  76.47 &       - &      - &      - &    100 \\
5382 &      - &   80 &      - &      - &      - &      - &    - &      - &      - &       - &      - &  33.34 &      - \\
5478 &  67.86 &    - &      - &      - &      - &      - &    - &      - &      - &       - &      0 &      - &      - \\
5540 &      - &    - &      - &      - &      - &  83.34 &    - &      - &      - &       - &      - &      - &    100 \\
5568 &      - &    - &      - &      - &      - &      - &    - &      - &      - &   85.71 &      - &      - &    100 \\
5664 &    100 &    - &      - &    100 &      - &      - &    - &      - &      - &       - &      - &    100 &      - \\
6020 &      - &    - &  66.67 &      - &      - &  57.14 &    - &      - &      - &       - &      - &      - &      - \\
6084 &      - &    0 &  62.81 &      0 &      - &     50 &  100 &      - &      - &       - &    100 &      - &  57.14 \\
6104 &      - &    0 &      - &      - &      - &      - &  100 &     50 &      - &       - &     50 &      - &      - \\
6168 &      - &    - &      - &      - &      - &      - &    - &      - &      - &       - &      - &      - &      - \\
6218 &      - &   40 &      - &      - &      - &    100 &    - &      - &      - &       - &      - &      0 &      - \\
6263 &      - &    - &    100 &      - &      - &      - &  100 &      - &      - &       0 &      - &      - &      - \\
6481 &    100 &   50 &      0 &  33.33 &      - &  61.89 &    0 &     80 &      - &       - &     50 &     50 &      - \\
6628 &      - &    - &     50 &      - &      - &    100 &    - &      - &      - &       - &      - &     50 &      - \\
6653 &  99.99 &    - &      - &      - &      - &      - &    0 &      - &      - &       - &      - &      - &    100 \\
6690 &      - &    - &  66.66 &      - &      - &      - &    - &      - &  53.34 &       - &      - &      - &      - \\
6709 &      - &    - &      - &    100 &      - &      - &    - &    100 &      - &       - &      - &  64.28 &      - \\
6717 &      - &    - &      - &      - &      - &      - &    - &      - &      - &       - &      - &      - &      - \\
6939 &      - &   75 &      - &      - &      - &    100 &    - &      - &      - &       - &      - &      - &      - \\
7187 &      - &   60 &      - &      - &      - &      - &    - &      - &      - &      50 &      - &      - &  68.42 \\
7409 &      - &    - &      - &      - &      - &      - &    - &    100 &      - &       - &      - &      - &      - \\
7424 &     50 &    0 &  66.66 &      - &  69.38 &    100 &    - &     50 &  33.34 &     100 &      - &      - &      - \\
7614 &      - &    0 &  68.43 &      - &      - &      - &    - &      - &      - &       - &      - &      - &      - \\
7650 &      - &  100 &      - &      - &      - &      - &    - &      - &      - &       - &      - &      - &      - \\
7906 &      0 &   50 &      - &  76.47 &  86.41 &      - &    - &     50 &      - &       - &     50 &  66.66 &      0 \\
8322 &      - &  100 &      - &      - &  79.22 &      - &    - &      - &      0 &       - &    100 &      - &      - \\
8507 &      - &    - &      - &      - &      - &      - &    - &      - &      - &       - &      0 &      - &      - \\
\bottomrule
\end{tabularx}
\end{table*}
